Meta-SGD: Learning to Learn Quickly for Few-Shot Learning

Few-shot learning is challenging for learning algorithms that learn each task in isolation and from scratch. In contrast, meta-learning learns from many related tasks a meta-learner that can learn a new task more accurately and faster with fewer examples, where the choice of meta-learners is crucial. In this paper, we develop Meta-SGD, an SGD-like, easily trainable meta-learner that can initialize and adapt any differentiable learner in just one step, on both supervised learning and reinforcement learning. Compared to the popular meta-learner LSTM, Meta-SGD is conceptually simpler, easier to implement, and can be learned more efficiently. Compared to the latest meta-learner MAML, Meta-SGD has a much higher capacity by learning to learn not just the learner initialization, but also the learner update direction and learning rate, all in a single meta-learning process. Meta-SGD shows highly competitive performance for few-shot learning on regression, classification, and reinforcement learning.

==> Results.tex <==
The base-learner in our experiment consists of 4 convolutional modules
and two fully connected modules. Each convolutional module is 
with $3\times
3$ convolutions and 64 filters,  followed by batch
normalization~\cite{ioffe2015batch}, a ReLU nonlinearity, and $2\times
2$ max-pooling. In our experiment, the size of image is $84\times 84$,
thus the dimension of the last module is $1600$. The first fully
connected module consists of one $1600\times
800$ linear layer, followed by batch normalization and a ReLU
nonlinearity. The last fully connected module includes one $800\times
5$ linear layer, followed by softmax nonlinearity. 
Finally there are two fully connected linear layers followed by
soft-max for the number of classes.

Note that our network has more
than $10^6$ parameters, which is much larger than the network used in
\cite{ravi2017optimization,finn2017model}. We also attempt to adopt
\citet{ravi2017optimization} to optimize over the same network for
comparison. However, Meta-Learner LSTM \citep{ravi2017optimization}
is not scalable to such large network.
In our approach,  $\thetab_1$ contains the weights
of all the convolutional layers and the first fully connected linear
layer, while $\thetab_2$ contains the weights of the second fully
connected linear layer.
It is notable that $\thetab_2$ has only 4005 parameters, which means that the
input size of LSTM can  be significantly reduced. Thus our approach is
scalable to larger networks. 
%When both shared weights ${\thetab}_1$ and task-specific weights ${\thetab}_2$ are present, we also employ a powerful external CNN network, from which ${\thetab}_1$ are derived, and append to the external network a final fully connected linear layer whose parameters form ${\thetab}_2$.
In our implementation, the state size of LSTM is 200.
%To compare our model with MAML~\cite{finn2017model}, we also run experiments for the small CNN network with fixed step size. We tested various values for the step size and report only the best result which is achieved at $0.4$.


\begin{table}[t]
	\centering
	\begin{center}
		\caption{Experimental Results on miniImageNet and ImageNet}
		\label{tab:res_miniImgNet}
		\begin{tabular}{|l|c|c|c|c|}
			\hline
			\multirow{2}{*}{Omniglot~\cite{lake2011one}} & \multicolumn{2}{c|}{5-way Accuracy} & \multicolumn{2}{c|}{20-way Accuracy} \\ \cline{2-5}
			
			& 1-shot & 5-shot & 1-shot & 5-shot \\ \hline
			
			Siamese Nets~\cite{koch2015siamese} & $97.3\%$ & $98.4\%$ & $88.2\%$ & $97.0\%$ \\ \hline
			
			Matching Nets~\cite{vinyals2016matching} & $98.1\%$ & $98.9\%$ & $93.8\%$ & $98.5\%$ \\ \hline
			
			MAML~\cite{finn2017model} & $98.7 \pm 0.4 \% $ & $99.9 \pm 0.1 \% $ & $95.8 \pm 0.3 \% $ & $98.9 \pm 0.2 \% $ \\ \hline
			
			MAML (1 step)~\cite{finn2017model} & $99.1 \pm 0.39 \% $ & $99.5 \pm 0.2 \% $ & $95.2 \pm 0.4 \% $ & $98.4 \pm 0.1 \% $ \\ \hline
			
			Meta-SGD (ours) & $\mathbf{99.53 \pm 0.26 \%} $ & $\mathbf{99.93 \pm 0.09 \%} $ & $\mathbf{95.93 \pm 0.38 \%} $ & $\mathbf{98.97 \pm 0.19 \%} $ \\ \hline
			
		\end{tabular}
		
		\vspace{10pt}
		
		\begin{tabular}{|l|c|c|}
			\hline
			\multirow{2}{*}{MiniImagenet~\cite{ravi2017optimization}} & \multicolumn{2}{c|}{5-way Accuracy} \\ \cline{2-3}
			
			& 1-shot & 5-shot \\ \hline
			
			Matching Nets~\cite{vinyals2016matching} & $43.56 \pm 0.84 \% $ & $55.31 \pm 0.73 \% $ \\ \hline
			
			Meta-LSTM~\cite{ravi2017optimization} & $43.44 \pm 0.77 \% $ & $60.60 \pm 0.71 \% $ \\ \hline
			
			MAML~\cite{finn2017model} & $48.70 \pm 1.84 \% $ & $63.11 \pm 0.92 \% $ \\ \hline
			
			MAML (1 step) \cite{finn2017model} & $44.40 \pm 1.68 \% $ & $61.11 \pm 1.00 \% $ \\ \hline
			Meta-SGD (ours) & $\mathbf{50.47 \pm 1.87 \%} $ & $\mathbf{64.03 \pm 0.94 \%} $ \\ \hline
			
		\end{tabular}
	\end{center}
\end{table}


Our model is compared to three state of the art few-shot learning
approaches, including Meta-Learner LSTM by~\citet{ravi2017optimization},
Matching Nets by~\citet{vinyals2016matching} and MAML by~\citet{finn2017model}.
The experimental results of meta-testing accuracy on miniImageNet and ImageNet are summarized in Table~\ref{tab:res_miniImgNet}. The accuracy is evaluated over 600 meta-testing tasks with 95\% confidence intervals.
The results of Meta-Learner LSTM and Matching Nets on miniImageNet come from~~\cite{ravi2017optimization}, while all other results are obtained from our experiments.
Our model achieved accuracy of 43.47\% and 60.96\% for 1-shot and 5-shot classification respectively.
Moreover, our model outperformed the state of the art methods on the ImageNet with 300 images per class.

%We compare the accuracy of our model according to the number of episodes during meta-training against existing models, as shown in Figure~\ref{fig:300Acc}. We set a checkpoint every 1000 episodes. The accuracy is evaluated on 100 meta-training tasks and 100 meta-validation tasks, respectively, at each checkpoint. For 1-shot classification, the accuracy of our model on meta-validation tasks is higher than that of other models at most data points, especially after 10000 episodes, although our accuracy on meta-training tasks is lower than Matching Nets. For 5-shot classification, the accuracy of our model is consistently higher than all other models, on both types of meta-training and meta-validation tasks.

%\begin{figure}
%	\centering
%%	\hspace{-50pt}
%	\begin{subfigure}[b]{0.38\textwidth}
%		\includegraphics[trim={0 0 1in 0},clip,width=\textwidth]{Results/plots/imgNet300AccLog1shot.pdf}
%		\caption{1-shot}
%		\label{fig:imgNet300Acc-1shot}
%	\end{subfigure}
%%	\hspace{-50pt}
%	\begin{subfigure}[b]{0.38\textwidth}
%		\includegraphics[trim={0 0 1in 0},clip,width=\textwidth]{Results/plots/imgNet300AccLog5shot.pdf}
%		\caption{5-shot}
%		\label{fig:imgNet300Acc-5shot}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.22\textwidth}
%		\includegraphics[trim={0 0in 0 0},clip,width=\textwidth]{Results/plots/imgNet300AccLogLegend.pdf}
%%		\caption{legend}
%		\label{fig:imgNet300Acc-legend}
%	\end{subfigure}
%	\caption{Comparison of various models' accuracy on meta-training tasks and meta-validation tasks. Dashed lines represent accuracy on meta-training tasks, and solid lines represent accuracy on meta-testing tasks.}\label{fig:300Acc}
%\end{figure}

%\begin{figure}
%	\centering
%	%	\hspace{-50pt}
%	\begin{subfigure}[b]{0.38\textwidth}
%		\includegraphics[trim={0 0 1in 0},clip,width=\textwidth]{Results/plots/imgNet300LossLog1shot.pdf}
%		\caption{1-shot}
%		\label{fig:imgNet300Loss-1shot}
%	\end{subfigure}
%	%	\hspace{-50pt}
%	\begin{subfigure}[b]{0.38\textwidth}
%		\includegraphics[trim={0 0 1in 0},clip,width=\textwidth]{Results/plots/imgNet300LossLog5shot.pdf}
%		\caption{5-shot}
%		\label{fig:imgNet300Loss-5shot}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.20\textwidth}
%		\includegraphics[trim={0 0.8in 0 0},clip,width=\textwidth]{Results/plots/imgNet300LossLogLegend.pdf}
%		%		\caption{legend}
%		\label{fig:imgNet300Loss-legend}
%	\end{subfigure}
%	\caption{Comparison of various models' loss on meta-training tasks and meta-validation tasks}\label{fig:300Loss}
%\end{figure}


%\begin{table}[h]
%	\caption{Experimental Results on Omniglot}
%	\label{table:res_omniglot}
%	\centering
%	\begin{tabular}{|c|c|c|c|c|}
%		\hline
%		\multirow{2}{*}{Training Settings} & 	\multicolumn{2}{ c| }{5-way Accuracy} & \multicolumn{2}{ c| }{20-way Accuracy} \\
%		\cline{2-5}
%		& 1-shot & 5-shot & 1-shot & 5-shot \\
%		\hline
%		Meta-Learner LSTM~\cite{ravi2017optimization} & & & & \\
%		\hline
%		Matching Nets~\cite{vinyals2016matching} & 98.1\% & 98.9\% & 93.8\% & 98.5\% \\
%		\hline
%		MAML~\cite{finn2017model} & $98.7 \pm 0.8\%$ & $99.9 \pm 0.3\%$ & $93.1 \pm 1.5\%$ & $98.8 \pm 0.6\%$ \\
%		\hline
%		Ours & & & & \\
%		\hline
%	\end{tabular}
%\end{table}


\begin{figure}[h]
  \centering
  \begin{subfigure}{0.32\textwidth}
  	\centering
  	%\vspace{-4pt}
  	\includegraphics[width=\textwidth]{figures/Generalize.pdf}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
  	\centering
  	\includegraphics[width=\textwidth]{figures/SLvsS.pdf}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
  	\centering
  	\includegraphics[width=\textwidth]{figures/LossVsS.pdf}
  \end{subfigure}

  \caption{Behavior of our meta-learner. {\bf Left:}
 Comparison of generalization ability. All four meta-learners are
 trained using 5-shot episodes, and tested using both 1-shot and
 5-shot episodes.     {\bf Middle:} Typical learned
    step-length $\alpha_t$. {\bf Right:} Typical training and testing
    loss on a 5-shot episode sampled from ImageNet.}
  \label{fig:Opt_Behavi}
\end{figure}

We consider how well the models generalize to situations where the number of shots in meta-training tasks and meta-testing tasks are different. As shown in Figure~\ref{fig:Opt_Behavi}, our model achieves accuracy of 48.19\% when trained with 5-shot episodes and tested with 1-shot tasks. Matching Nets has higher accuracy for 1-shot testing, but relatively low accuracy in the 5-shot case. Overall our model performs well when training and testing tasks have the same number of shots, and has good generalization ability at the same time.
We also visualize the changing process of learning rate, training loss and testing loss within a typical episode in Figure~\ref{fig:Opt_Behavi}. The learning rate learned by LSTM decreases as training proceeds, which shows the effectiveness of learning this learning rate. The training loss and testing loss drops greatly after two steps, and afterwards training loss drops gradually while testing loss remains almost the same. This gives evidence that to achieve high testing accuracy the training process needs to proceed for at least two steps, while further steps may provide marginal gain to the accuracy.

% Added by Zhen, so that latex can identify which is the main file
%%% Local Variables:
%%% TeX-master: "nips_2017"
%%% End:


==> bib.tex <==
\section*{References}

References follow the acknowledgments. Use unnumbered first-level
heading for the references. Any choice of citation style is acceptable
as long as you are consistent. It is permissible to reduce the font
size to \verb+small+ (9 point) when listing the references. {\bf
  Remember that you can go over 8 pages as long as the subsequent ones contain
  \emph{only} cited references.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms
for connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and
T.K.\ Leen (eds.), {\it Advances in Neural Information Processing
  Systems 7}, pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS:
  Exploring Realistic Neural Models with the GEneral NEural SImulation
  System.}  New York: TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of
learning and recall at excitatory recurrent synapses and cholinergic
modulation in rat hippocampal region CA3. {\it Journal of
  Neuroscience} {\bf 15}(7):5249-5262.

==> motivation.tex <==
%\subsection{Meta-Learning}

%Let us first clarify the notations. To specify a base-learner $f_{\thetab}$, we need to determine its type and parameters. So $CNN_{\thetab}$ refers to a convolutional neural network (CNN) as the type of the base-learner and its weights $\thetab$ as the parameters. Similarly, $M$ denotes the type of the meta-learner and $\phib$ the corresponding parameters.

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\textwidth]{figures/learning.pdf}
%	\caption{\small Illustrating how a meta-learner adapts a template base-learner using a few examples for a new task. The meta-learner first initializes the template base-learner with task-shared weights $\thetab_1$ and task-specific weights $\thetab_2=\thetab_2^0$, and then updates the task-specific weights $\thetab_2$ using gradient descent with learning rate $\alpha$ provided by a learned LSTM for $T$ steps. Specifically, in step $t$, the LSTM takes as input the current task-specific weights $\thetab_{2,i}^{t-1}$, loss $\mathcal{L}_i^t$ and gradient $\nabla_{\thetab_{2}} \mathcal{L}_i^t$, and outputs a learning rate $\alpha^t$, to update $\thetab_{2,i}^{t}=\thetab_{2,i}^{t-1}-\alpha^t \nabla_{\thetab_{2}} \mathcal{L}_i^t(\thetab_1,\thetab_{2,i}^{t-1})$. The prediction loss $\mathcal{L}_i^{test}$ is used to update the meta-learner using BPTT.}
%	\label{fig:learning_algorithm}
%\end{figure}

\subsection{Motivation}
Given a learner $f_{\thetab}$, how can a meta-learner $M_{\phib}$ adapt it for a new task from a few examples $D=\{(\xb_i,\yb_i)\}$?
One standard method is by gradient descent to update the model as follows:
\begin{equation}\label{euq:typical_updates}
\thetab^{t}  = \thetab^{t-1} - \alpha^{t} \nabla\mathcal{L}_D(\thetab^{t-1}).
\end{equation}
Here, $\nabla\mathcal{L}_D$ is the gradient of the empirical loss $\mathcal{L}_D(\thetab)= \frac{1}{|D|}\sum_{(\xb,\yb)\in D} \ell(f_{\thetab}(\xb), \yb)$, and $\alpha^{t}$ is the learning rate at step $t$. Besides the learning rate at each step, one also needs to specify the initial parameters $\thetab^0$. Usually, these parameters are hand-crafted and the iterative learning process continues until the empirical loss is minimized. This may be feasible with a large amount of labeled data, but it is prone to overfitting with small data. 

%One typical way to address overfitting is by regularization. However, with only a few examples, traditional methods of imposing regularization over the model parameters such as $L^2$ norm will not ensure good performance on new examples. Another way is to use transfer learning which relies on previously trained models. Its performance depends on how relevant of the previous model to the task of interest~\cite{yosinski2014transferable}. In either way, the goal is in relying on certain inductive bias to guide the process of learning. We need a principled way to acquire and encode a strong yet accurate inductive bias, as well as a systematic way to use it to guide the few-shot learning task at hand.

% that can produce a good initialization of parameters and updating rules. The base-learner itself may have the ability to extract meta-level inductive bias although it is designed for task solving. This motivates us to design a new structure for the base-learner.

%In the perspective of learning-to-learn, one can learn such inductive bias, as well as the way in guiding the learning process.
In what follows, we will present our method for learning how to learn a high-capacity deep model from many related tasks, including how to encode the inductive bias, the initialization, and the learning rate at each step. The proposed learning process is illustrated in Figure~\ref{fig:learning_algorithm}.

\begin{figure}[t]
	\centering
	\includegraphics[width=\textwidth]{figures/learning.pdf}
	\caption{\small Illustrating how a meta-learner adapts a template base-learner using a few examples for a new task. The meta-learner first initializes the template base-learner with task-shared weights $\thetab_1$ and task-specific weights $\thetab_2=\thetab_2^0$, and then updates the task-specific weights $\thetab_2$ using gradient descent with learning rate $\alpha$ provided by a learned LSTM for $T$ steps. Specifically, in step $t$, the LSTM takes as input the current task-specific weights $\thetab_{2,i}^{t-1}$, loss $\mathcal{L}_i^t$ and gradient $\nabla_{\thetab_{2}} \mathcal{L}_i^t$, and outputs a learning rate $\alpha^t$, to update $\thetab_{2,i}^{t}=\thetab_{2,i}^{t-1}-\alpha^t \nabla_{\thetab_{2}} \mathcal{L}_i^t(\thetab_1,\thetab_{2,i}^{t-1})$. The prediction loss $\mathcal{L}_i^{test}$ is used to update the meta-learner using BPTT.}
	\label{fig:learning_algorithm}
\end{figure}



%\begin{wrapfigure}{r}{0.5\textwidth}
%	\vspace{-15pt}
%	\begin{center}
%		\includegraphics[width=0.48\textwidth]{figures/LSTM.pdf}
%	\end{center}
%	%	\vspace{-10pt}
%	\caption{The structure of the used ${LSTM}_{\phib}$. The $t$-th step outputs a learning rate $\alpha^t = \beta\cdot \sigma(\wb^\top\hb^t+b)$ based on hidden state $\hb^t$, where $\beta>0$ is a scaling factor, and $\wb$ and $b$ are the corresponding parameters of ${LSTM}_{\phib}$.}
%	\vspace{-10pt}
%	\label{fig:lstm}
%\end{wrapfigure}


==> our-model.tex <==
\input{motivation}




%There are two issues worth considering: how to determine the number of steps and how to choose the learning rate $\alpha^{t}$ for each step. When we do not have sufficiently many examples for $D$, the optimal $\thetab^*$ will easily lead to the overfitting of our model on $D$.
%Hence, with limited number of training examples for each task, the number of steps cannot be too large and the goal of updating the learner's parameters is to minimize the loss functions with respect to the examples in $D_{test}(P_i)$.

\subsection{Method}
We propose to learn a so-called neural composite network (NCN, Figure~\ref{fig:controller}) as a base-learner, which is composed of (task-)shared weights $\thetab_1$ across tasks and task-specific weights $\thetab_2$. This is inspired by the biological evidence that changes in synaptic efficacy occur in different time-scales~\cite{kupfermann1979modulatory,hartzell1981mechanisms}. Take a deep CNN as a base-learner,
the first several convolution layers can serve as the task-shared weights, while the final few fully connected layers as task-specific weights. We expect the task-shared weights $\thetab_1$ of the base-learner ($f_{\thetab_1, \thetab_2}$) to capture task-agnostic meta-level knowledge, which can guide the meta-learner in updating the task-specific weights $\thetab_2$ for a new task using a few examples. Consequently, the meta-learner should slowly learn the task-shared weights from many related tasks and quickly learn the task-specific weights in the neural network in a joint learning process. It should also learn how to initialize the base-learner and control the rate of learning.

%More specifically, the task-specific weights of the NCN are rapidly updated by a meta-learner to capture task-level information while the shared weights are slowly updated by gradient descent to accumulate meta-level inductive bias, in a single learning process. Importantly, the meta-learner also learns to initialize the learning of the base-learner and control the subsequent learning rates.
%Upon a few-shot learning task, the meta-learner only needs to update the task-specific weights of the NCN in the learned manner and thus is very efficient.

\begin{figure}[h]
%	\vspace{-15pt}
	\begin{center}
		\includegraphics[width=0.5\textwidth]{figures/LSTM.pdf}
	\end{center}
	%	\vspace{-10pt}
	\caption{The structure of the used ${LSTM}_{\phib}$. The $t$-th step outputs a learning rate $\alpha^t = \beta\cdot \sigma(\wb^\top\hb^t+b)$ based on hidden state $\hb^t$, where $\beta>0$ is a scaling factor, and $\wb$ and $b$ are the corresponding parameters of ${LSTM}_{\phib}$.}
%	\vspace{-10pt}
	\label{fig:lstm}
\end{figure}

%According to this point of view, how to update $\thetab_{i}^{t}$ is somehow dependent on all the tasks.
Motivated by previous works~\cite{cotter1990fixed,younger1999fixed,hochreiter2001learning,andrychowicz2016learning,ravi2017optimization}, we use $LSTM_{\phib}$ to learn an update rule for the learning rate $\alpha_t$ for gradient descent and thus, provide an update rule for the base-learner according to Eq.~\eqref{euq:typical_updates}.
%It is known that recurrent neural networks (RNNs) have the capacity to simulate arbitrary procedures since they are Turing-complete~\cite{siegelmann1992computational}, and a crucial innovation to RNNs is the Long Short-Term Memory (LSTM). The dynamic cell state in LSTM can mimic the moving average of input and capture the long-term dependency. There are some similar architectures to LSTM, and we use LSTM here because of its good performance in practice.
%\textbf{Meta-Learner.}
Specifically, the learning rate $\alpha_{i}^{t}$ and the parameters $\thetab_{2,i}^{t}$ are updated as follows:
\begin{align}
& \alpha_{i}^{t} = LSTM_{\phib}(\thetab_{2,i}^{t-1}, \mathcal{L}_{D_{train}(P_i)}(\thetab_1, \thetab_{2,i}^{t-1}), \nabla_{\thetab_2}\mathcal{L}_{D_{train}(P_i)}(\thetab_1, \thetab_{2,i}^{t-1})), \label{euq:learning_rate_updates} \\
& \thetab_{2,i}^{t} = \thetab_{2,i}^{t-1} - \alpha_{i}^{t} \nabla_{\thetab_2}\mathcal{L}_{D_{train}(P_i)}(\thetab_1, \thetab_{2,i}^{t-1}). \label{euq:parameters_updates}
\end{align}

We use a single-layer LSTM network with a standard structure inside, illustrated in Figure~\ref{fig:lstm}. The network takes as input the current parameter value $\thetab_{2,i}^{t-1}$, the current loss $\mathcal{L}_{D_{train}(P_i)}(\thetab_1, \thetab_{2,i}^{t-1})$ on the training set $D_{train}(P_i)$, the current gradient $\nabla_{\thetab_2}\mathcal{L}_{D_{train}(P_i)}(\thetab_1, \thetab_{2,i}^{t-1})$ with respect to parameters $\thetab_2$, as well as the previous hidden state $\hb^{t-1}$, and outputs the update for the next learning rate $\alpha_t$. While other choices of input are possible, we regard the learning rate as a function of the moving average of parameters, loss function, and gradient of the loss function inspired by some previous successful optimization methods used in deep learning, such as Adagrad~\cite{duchi2011adaptive} and RMSprop~\cite{tieleman2011adaptive} which scale the learning rate based on $L^2$ norm of all previous gradients, Adam~\cite{kingma2014adam} which scales the learning rate based on both previous gradients and $L^2$ norm of them, and Adadelta~\cite{zeiler2012adadelta} which additionally includes the expected squared change of parameters. Polyak's method~\cite{polyak1969minimization} suggests that we shall also consider the value of the loss function. Our design of input is a balance between expressivity and complexity.

%The training of NCN as a base-learner is illustrated in Figure~\ref{fig:learning_algorithm}.

%Here, we use the following variant of the LSTM architecture:
%\begin{equation}
%\begin{split}
%\ib^t &= \sigma(W_{\ib}[\boldsymbol{\chi}^{t}; \hb^{t-1}]+\bb_{\ib}) \\
%\fb^t &= \sigma(W_{\fb}[\boldsymbol{\chi}^{t}; \hb^{t-1}]+\bb_{\fb}) \\
%\ob^t &= \sigma(W_{\ob}[\boldsymbol{\chi}^{t}; \hb^{t-1}]+\bb_{\ob}) \\
%\cb^t &= \fb^t\cb^{t-1} + \ib^t\tanh(W_{\cb}[\boldsymbol{\chi}^{t}; \hb^{t-1}]+\bb_{\cb}) \\
%\hb^t &= \ob^t\tanh(\cb^t) \\
%\alpha_i^t &= \sigma(\wb^\top\hb^t+b)
%\end{split}
%\end{equation}
%where $\boldsymbol{\chi}^{t}=[\thetab_{2,i}^{t-1}; \nabla_{\thetab_{2,i}^{t-1}}\mathcal{L}_{D_{train}(P_i)}(\thetab_1, \thetab_{2,i}^{t-1}); \mathcal{L}_{D_{train}(P_i)}(\thetab_1, \thetab_{2,i}^{t-1})]$.






%%% Local Variables:
%%% TeX-master: "nips_2017"
%%% End:





==> problem-statement.tex <==

\section{Preliminaries on Learning to Learn}\label{sec:l2l}
%To
%
%
%\zzhang{I have some concerns about the notations. Usually the input of
%  $f$ are not scalar, so that shall we use $\xb$ and $\yb$ instead of
%  $x$ and $y$. Also the parameters of learner and meta-learner are not
%  scalar,
%  so that shall we use $\thetab$ and $\phib$ instead?
%}
%\zhenguo{This is a good point. Fengwei may modify accordingly. }


In the problem of learning-to-learn, we have two learners, a meta-learner and a base-learner. The meta-learner learns from many related tasks how to learn a base-learner.
%the process of which is often referred as meta-learning.
In the case of few-shot learning, the meta-learner should learn the base-learner using only a few examples.
%Our goal is to train such a meta-learner.
%Let $X$ be an input space and $Y$ an output space.
%A learning task is represented by a probability distribution $P$ on $X\times Y$ and
Mathematically, a base-learner is a mapping from an input space $X$ to an output space $Y$, while
a meta-learner is a mapping from the power set of $X\times Y$ to the base-learner hypothesis space.
Denote by $f_{\thetab}:X\rightarrow Y$ a base-learner parameterized by $\thetab$. Varying $\thetab$ gives a base-learner hypothesis space, $\mathcal{H}=\{f_{\thetab}\}$.
Denote by $M_{\phib}: \mathbb{P}(X\times Y)\rightarrow \mathcal{H}$ a meta-learner parameterized by $\phib$, where $\mathbb{P}(X\times Y)$ denotes the power set of $X\times Y$, i.e., the set of all subsets of $X\times Y$. Our task is to find a meta-learner $M_{\phib}$ and a template base-learner $f_{\thetab}$ such that $M_{\phib}$ can quickly adapt $f_{\thetab}$ using a few examples.

%$\mathbb{P}(X\times Y)$\footnote{The set of all subsets of $X\times Y$.}

More specifically, consider a meta-learning task dataset $\mathcal{D}$ with $n$ tasks $P_1, P_2, \cdots, P_n$. For simplicity, assume each task consists of $m=m_1+m_2$ labeled examples sampled from an unknown probability distribution over $X\times Y$, divided into a training set of size $m_1$ and a testing set of size $m_2$. The meta-learning task can be formulated as an optimization problem:
\begin{equation}\label{euq:meta-learning_obj}
  % modified by Zhen
  % We have a particular symbol \ell for loss
\min_{\phib, \thetab}\ \frac{1}{n}\sum_{i=1}^{n}\,\frac{1}{m_2}\sum_{(\xb,\yb)\in D_{test}(P_i)} \ell(M_{\phib}(D_{train}(P_i)|f_{\thetab})(\xb), \yb),
\end{equation}
where $\ell:Y\times Y\rightarrow \mathbb{R}$ is a loss function, and $D_{train}(P_i)$ and $D_{test}(P_i)$ denote the training and testing sets of task $P_i$, respectively. $M_{\phib}(D_{train}(P_i)|f_{\thetab})$ refers to the process the meta-learner $M_{\phib}$ adapts the template base-learner $f_{\thetab}$ to give a desired base-learner, using a few examples $D_{train}(P_i)$.

%Actually, the meta-learner $M_{\phib}$ provides an adaptive optimization algorithm for updating the parameters of the learner $f_{\thetab}$ according to the training set of each task. We will discuss it in detail in the following subsections.




==> train.tex <==
%\subsection{Meta-Training}

\subsection{Meta-Training}
Let $\thetab_{2,i}^0$ be $\thetab_2^0$ for every task $P_i$ and fix the
number of steps $T$. Then, the final form of the base-learner $f_{\thetab_1,\thetab_{2,i}^{T}}$, denoted by $M_{\phib}(D_{train}(P_i)|f_{\thetab_1,\thetab_2^0})$, depends on the meta-level parameters $\thetab_1$, $\thetab_2^0$, and $\phib$. Our
meta-learning task can be formulated as the following optimization problem:
%\zzhang{From current notation, it is not clear that $\theta_2$ in
%  \eqref{euq:meta-learning_obj_new} is the initial value of
%  $\theta_{2i}$ in \eqref{euq:typical_updates}}
\begin{equation}\label{euq:meta-learning_obj_new}
\min_{\phib, \thetab_1, \thetab_2^0}\
\frac{1}{n}\sum_{i=1}^{n}\,\frac{1}{m_2}\sum_{(\xb,\yb)\in D_{test}(P_i)} \ell(M_{\phib}(D_{train}(P_i)|f_{\thetab_1,\thetab_2^0})(\xb), \yb).
\end{equation}
The stochastic gradient descent (SGD) algorithm can be applied to optimize 
the problem in Eq.~\eqref{euq:meta-learning_obj_new}, where the gradient is
computed via the Back-Propagation Through Time (BPTT) algorithm~\citep{werbos1990backpropagation}. In particular, in our implementation, we
use the Adam~\citep{kingma2014adam} method, a variant of SGD. The overall meta-training process is summarized in Algorithm~\ref{algo:train}.

\IncMargin{1.5em}
\begin{algorithm}[t]\small
	\caption{\small Meta-Training}
	\label{algo:train}
	\SetNlSty{textbf}{}{:}
	\SetAlgoNoLine
	
	\Indm
	\KwIn{Meta-learning dataset with $n$ tasks $\mathcal{D}=\{P_i\}_{i=1}^n$
            %base-learner $f$
          %parameterized by $\thetab_1$ and $\thetab_2$, meta-learner
          %$M$ parameterized by $\phib$,.
	}
	\KwOut{$M_{\phib},\ f_{\thetab_1, \thetab_2^0}$
	}

	\Indp
	randomly initialize $\phib, \thetab_1, \thetab_2^0$\;
	\For{$i = 1,\ldots, n$}{
		%sample $D_{train}(P_i)$ and $D_{test}(P_i)$ for task $P_i$ from $\mathcal{D}$\;
		$\thetab_{2,i}^0 \leftarrow \thetab_2^0$\;
		\For{$t = 1,\ldots, T$}{
			$\mathcal{L}_{i}^t \leftarrow \frac{1}{|D_{train}(P_i)|}\sum_{(\textbf{x}, \textbf{y}) \in D_{train}(P_i)} \ell(f_{\thetab_1, \thetab_{2,i}^{t-1}}(\textbf{x}), \textbf{y})$\;
			$\alpha_{i}^{t} \leftarrow LSTM_{\phi}(\thetab_{2,i}^{t-1}, \mathcal{L}_{i}^t, \nabla_{\thetab_2} \mathcal{L}_i^t)$\;
			$\thetab_{2,i}^t \leftarrow \thetab_{2,i}^{t-1} - \alpha_i^t \nabla_{\thetab_2} \mathcal{L}_{i}^t$\;
		}
		$\mathcal{L}_i^{test} \leftarrow
                \frac{1}{|D_{test}(P_i)|}\sum_{(\textbf{x},
                  \textbf{y})\in D_{test}(P_i)} \ell(f_{\thetab_1,
                  \thetab_{2,i}^{T}}(\textbf{x}), \textbf{y})$\;

                $(\phib, \thetab_1, \thetab_2^0) \leftarrow (\phib,
                \thetab_1, \thetab_2^0) - \gamma \nabla \mathcal{L}_i^{test}(\phi,
                  \thetab_1, \thetab_2^0)$ \;

		% update $\phib$, $\thetab_1$ and $\thetab_2^0$ using $\nabla_{(\phi, \thetab_1, \thetab_2^0)} \mathcal{L}_i^{test}$
	}
	
\end{algorithm}


%%% Local Variables:
%%% TeX-master: "nips_2017"
%%% End:


==> unified-view.tex <==
%\subsection{Comparison with Related Work}

\subsection{A Unified View}
%to relate four existing models: matching network, model-agnostic meta-learning, optimization as a model, and meta network
Interestingly, our learning-to-learn method can be seen as a framework for few-shot learning. Different structures of meta-learner and base-learner, and different encodings of meta-level and task-specific knowledge in a base-learner may lead to different models. In what follows, we discuss how several existing models are related in this framework.

\textbf{Meta-Learner LSTM~\cite{ravi2017optimization}.}
If we do not model the task-shared weights $\thetab_1$ in our base-learner, then the task-specific weights $\thetab_2$ take the place of the whole weights $\thetab$ and our meta-learning problem reduces to
\begin{equation}\label{euq:meta-learning_obj_without_slow_weights}
\min_{\phib, \thetab^0}\
\frac{1}{n}\sum_{i=1}^{n}\,\frac{1}{m_2}\sum_{(\xb,\yb)\in D_{test}(P_i)} \ell(M_{\phib}(D_{train}(P_i)|f_{\thetab^0})(\xb), \yb),
\end{equation}
which is essentially the Meta-Learner
LSTM~\cite{ravi2017optimization}. The only difference is in the update
rule of $\thetab$. Their model uses the cell state of an LSTM to
represent $\thetab$ and regards $\thetab^0$ as the initial cell state,
while ours updates $\thetab$ by gradient descent with adaptive
learning rates learned by the LSTM and $\thetab^0$ is learned across
related tasks. In order to optimize a deep Convolutional Neural
Network (CNN) with tens of thousands of parameters, their method operates coordinate-wise on the parameters by the same LSTM-based meta-learner. In contrast, our method divides the parameters into task-shared weights and task-specific weights, and the meta-learner only needs to update the latter.

The main limitation of Meta-Learner LSTM lies in its scalability. Only after the LSTM outputs the final parameter of the base-learner, the meta-training prediction loss can be evaluated. As a result, the Back-Propagation Through Time (BPTT)~\citep{werbos1990backpropagation} method is used to compute the gradient of the meta-learner parameters. However, BPTT requires to store all intermediate results of the LSTM, which has a space complexity of $\Ocal(T\#(states)\text{dim}(\thetab))$ with $T$ as number of time steps, $\#(states)$ as number of states in LSTM and $\text{dim}(\thetab)$ as number of parameters in the learner. A typical number of $T$ is $8$, and $20$ for $\#(states)$. Furthermore, due to the complicated computations inside LSTM, the constant factor for the complexity $\Ocal(T\#(states)\text{dim}(\thetab))$ can also be large, which indicates that Meta-Learner can not scale up to large networks.

%Their coordinatewise updating method overlooks the correlation among parameters and using the same updating rule on each coordinate gives no consideration to the difference among different types of layers. Our method, in contrast, takes the integrated information of parameters and loss functions into account and regards the parameters of convolution layers as the shared parameters across tasks that may capture the meta-level inductive bias.
%Since the same update rule is used independently on each coordinate, their model
%to prevent an explosion of meta-learner parameters




\textbf{Model-Agnostic Meta-Learning~\cite{finn2017model}.}
Similarly, if we do not model the task-shared weights $\thetab_1$ in our base-learner, and in the gradient descent of $\thetab_2$ we use a constant learning rate $\alpha$, i.e., $\thetab_{2,i}^{t}  = \thetab_{2,i}^{t-1} - \alpha \nabla\mathcal{L}_{D_{train}(P_i)}(\thetab_{2,i}^{t-1})$, then our model reduces to the Model-Agnostic Meta-Learning (MAML)~\cite{finn2017model}. This method has to tune the learning rate by hand, which can vary for each step and over a wide range for different problems. In our experiments, after a fine tuning of the learning rate, their method achieved a good performance.

%\textbf{Matching Nets~\cite{vinyals2016matching}.}
%If the learner does not contain the task-level fast weights $\thetab_2$, then our meta-learning problem objective reduces to
%\begin{equation}\label{euq:meta-learning_obj_without_fast_weights}
%\min_{\thetab_1}\
%\frac{1}{n}\sum_{i=1}^{n}\,\frac{1}{m_2}\sum_{(\xb,\yb)\in D_{test}(P_i)} \ell(f_{\thetab_1}(\xb), \yb).
%\end{equation}
%Moreover, for each task $P_i$, if we let the learner be
%\begin{equation}\label{euq:attention_matching}
%f_{\thetab_1}(\hat{\xb})=\sum_{(\xb,\yb)\in D_{train}(P_i)}a_{\thetab_1}(\hat{\xb}, \xb)\yb,
%\end{equation}
%where $a_{\thetab_1}(\hat{\xb}, \xb)=e^{c(g_{\thetab_1}(\hat{\xb}),\,g_{\thetab_1}(\xb))}/\sum_{(\xb,\yb)\in D_{train}(P_i)} e^{c(g_{\thetab_1}(\hat{\xb}),\,g_{\thetab_1}(\xb))}$, $g_{\thetab_1}$ is an embedding function and $c$ is the cosine distance, then our model reduces to Matching Nets in~\cite{vinyals2016matching}.

%If we discard the $LSTM_{\phib}$ and let the meta-learner $M_{\phib}$ be $M_{\phib}(D_{train}(P_i)|f_{\thetab_1,\thetab_2^0})=f_{\thetab_1, \thetab_{2,i}^{*}}$, where $\thetab_{2,i}^{*}  = \mathop{\arg\min}_{\thetab_2}\ \frac{1}{m_1}\sum_{(\xb,\yb)\in D_{train}(P_i)} \ell(f_{\thetab_1, \thetab_2}(\xb), \yb)$, then our model reduces to the model in~\cite{baxter1995learning,baxter2000model}. Indeed, their model does not divide the examples into two different sets for each task and their objective is
%\begin{equation}\label{euq:meta-learning_obj_without_LSTM}
%\min_{\thetab_1}\ \frac{1}{n}\sum_{i=1}^{n}\,\inf_{\thetab_2}\frac{1}{m}\sum_{(\xb,\yb)\in D(P_i)} \ell(f_{\thetab_1, \thetab_{2}}(\xb), \yb).
%\end{equation}
%When the number of training examples for each task is relatively small, their model may suffer from overfitting on the training set when facing a new task.








%%% Local Variables:
%%% TeX-master: "nips_2017"
%%% End:













